A generic approach to nonparametric function estimation with mixed data

In practice, data often contain discrete variables. But most of the popular nonparametric estimation methods have been developed in a purely continuous framework. A common trick among practitioners is to make discrete variables continuous by adding a small amount of noise. We show that this approach is justified if the noise distribution belongs to a certain class. In this case, any estimator developed in a purely continuous framework extends naturally to the mixed data setting. Estimators defined that way will be called continuous convolution estimators. They are extremely easy to implement and their asymptotic properties transfer directly from the continuous to the mixed data setting.

==> 3-regression.tex <==
\section{Jittering in regression models}

We saw in the previous section that, under a suitable choice of noise distribution, the joint densities in the original and jittered model coincide. As a consequence, we can hope that there are similar relationships for functionals of joint densities. This is very powerful, since most common regression-type problems can be formulated in terms of joint densities.

Generally speaking, regression models describe a conditional relationship between a \emph{response} variable and a vector of \emph{covariates} (also called \emph{predictors}). Let the response $Y \in \Omega_Y$  be either discrete or continuous and denote the vector of predictors as $(\bm Z, \bm X) \in \Z^p \times \R^q$. 

\begin{example}[Mean regression] \label{ex:mreg}
The conditional mean $\mathrm{E}(Y \mid \bm Z = \bm z, \bm X = \bm x)$ can be expressed as
\begin{align*}
\mu_{\bm z, \bm x}(f_{Y, \bm Z, \bm X}) =
\begin{cases}
 \bigl\{ \int_{\R} f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) ds \bigr\}^{-1} \int_{\R} s f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) ds, & \Omega_Y = \R, \\
\bigl\{ \sum_{s \in \Z} f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) \bigr\}^{-1} \sum_{s \in \Z} s f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) , &  \Omega_Y = \Z.
\end{cases}
\end{align*}
\end{example}

\begin{example}[Distribution regression] \label{ex:dreg}
The conditional distribution function $\Pr(Y \le y  \mid \bm Z = \bm z, \bm X = \bm x)$ can be expressed as
\begin{align*}
 \pi_{y \mid \bm z, \bm x}(f_{Y, \bm Z, \bm X}) = \begin{cases}
 \bigl\{ \int_{\R} f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) ds \bigr\}^{-1} \int_{-\infty}^y  f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) ds, & \Omega_Y = \R, \\
\bigl\{ \sum_{s \in \Z} f_{Y, \bm Z, \bm X}(s, \bm z, \bm x) \bigr\}^{-1} \sum_{s = - \infty}^y  f_{Y, \bm Z, \bm X}(s, \bm z, \bm x), &\Omega_Y = \Z.
\end{cases}
\end{align*}
\end{example}

\begin{example}[Quantile regression]
For $\alpha \in [0, 1]$, the conditional quantile function is defined as 
\begin{align*}
Q(\alpha \mid \bm z, \bm x) = \inf\bigl\{y \in \Omega_Y\colon\Pr(Y \le y  \mid \bm Z = \bm z, \bm X = \bm x) \ge \alpha  \bigr\},
\end{align*}
and can be expressed as
\begin{align*}
q_{y \mid \bm x, \bm z}(f_{Y, \bm Z, \bm X}) = \inf\bigl\{y \in \Omega_Y\colon  \pi_{y \mid \bm z, \bm x}(f_{Y, \bm Z, \bm X})  \ge \alpha  \bigr\},
\end{align*}
where $\pi_{y \mid \bm z, \bm x}$ is as in Example \ref{ex:dreg}. An important special case is \emph{median regression}, where $\alpha = 0.5$. 
\end{example}

\begin{example}[Classification]
Classification models are regression models where the response $Y$ is an unordered categorical variable, such as male/female or business sectors. They are characterized by the conditional class probabilities $\Prob(Y = y \mid\bm X =  \bm z, \bm X = \bm x)$, $y \in \Omega_Y$. It is possible to reformulate the classification model as a set of ordinary mean regressions, i.e.,
\begin{align*}
\Prob(Y = y \mid\bm X =  \bm z, \bm X = \bm x) = \mathrm{E}\bigl\{\ind(Y = y) \mid \bm Z = \bm z, \bm X = \bm x\bigr\}, \qquad y \in \Omega_Y.
\end{align*}
Hence, classification models can be seen as a special case of Example \ref{ex:mreg}.
\end{example}

In what follows, we shall use the notation of the previous section, where functionals of $f_{\bm Z, \bm X}$ (rather than $f_{Y, \bm Z, \bm X}$) were considered. To do this, we assign $Y$ to either $\bm Z$ or $\bm X$, depending on whether $Y$ is discrete or continuous. 

Suppose that the response variable $Y$ is continuous, set $Y = X_1$ and denote $\bm X_{-1} = (X_2, \dots, X_p)$. Then the regression models from the previous sections are characterized by functionals of the density $f_{\bm Z, \bm X}$. The following result is a direct consequence of the equality of the densities in the original and jittered model. It shows that  regression functions in the jittered model coincide with those in the original model.%, as illustrated in Fig.~\ref{cxmreg_ill}.
\begin{proposition}
If $\eta \in \mathcal{E}_{\gamma_1, \gamma_2}$ (as in Definition \ref{ce:BA_def}), it holds for all $(\bm z, \bm x) \in \Z^p \times \R^q$, $\alpha \in [0, 1]$,
\begin{align*}
\mu_{\bm z, \bm x_{-1}} (f_{\bm Z, \bm X}) &= \mu_{\bm z, \bm x_{-1}} (f_{\bm Z + \bm \epsilon, \bm X}), \\
 \pi_{x_1 \mid \bm z, \bm x_{-1}}(f_{\bm Z, \bm X}) &= \pi_{x_1 \mid \bm z, \bm x_{-1}}(f_{\bm Z + \bm \epsilon, \bm X}), \\ 
q_{\alpha \mid \bm z, \bm x_{-1}}(f_{\bm Z, \bm X}) &= q_{\alpha \mid \bm z, \bm x_{-1}}(f_{\bm Z + \bm \epsilon, \bm X}),
\end{align*}
\end{proposition}

%\begin{figure}
%	\centering
%    \subfloat[original data]{
%    \includegraphics[width = 0.315\textwidth]{fig/cxmreg_ill_1} 
%     \label{cxmreg_ill_1}
%     } 
%     \hspace{2cm}
%     \subfloat[continuously convoluted data]{
%    \includegraphics[width = 0.315\textwidth]{fig/cxmreg_ill_2}
%    \label{cxmreg_ill_2}
%    }  
%    \caption{Jittering in mean regression: observations (grey) and the true conditional mean (black).}
%    \label{cxmreg_ill}
%\end{figure}



Now suppose that the response variable $Y$ is discrete. By setting $Y = Z_1$, we see that the regression models are again functionals of $f_{\bm Z, \bm X}$. As the following result shows, they can be equivalently expressed as functionals of $f_{\bm Z + \bm \epsilon, \bm X}$. 

\begin{proposition} 
If $\eta \in \mathcal{E}_{\gamma_1, \gamma_2}$ (as in Definition \ref{ce:BA_def}), it holds for all $(\bm z, \bm x) \in  \Z^p \times \R^q$,  $\alpha \in [0, 1]$,
\begin{align*}
\mu_{\bm z_{-1},\bm x}(f_{\bm Z, \bm X}) &= \mu_{\bm z_{-1},\bm x}(f_{\bm Z + \bm \epsilon, \bm X}), \\
 \pi_{z_1 \mid \bm z_{-1}, \bm x}(f_{\bm Z, \bm X}) &= g_{\bm z, \bm x}(f_{\bm Z + \bm \epsilon, \bm X}), \\ 
q_{\alpha \mid \bm z_{-1}, \bm x}(f_{\bm Z, \bm X}) &= \inf\bigl\{z_1 \in \Z \colon g_{\bm z, \bm x}(f_{\bm Z + \bm \epsilon, \bm X}) \ge \alpha  \bigr\},
\end{align*}
where 
\begin{align*}
g(\bm z, \bm x) = \pi_{z_1 \mid \bm z_{-1}, \bm x}(f_{\bm Z + \bm \epsilon, \bm X}) + \frac{f_{\bm Z + \bm \epsilon, \bm X}(\bm z, \bm x) }{2 \int_{\R} f_{\bm Z + \bm \epsilon, \bm X}(\bm z, \bm x) dz_1}.
\end{align*}
\end{proposition}


Hence, any nonparametric estimator that consistently estimates a regression function in the continuous setting can be used to recover the corresponding function in a mixed data setting. We shall formalize this in the following section.

